Measurements of the Higgs boson production and decay rates and coupling strengths using $pp$ collision data at $\sqrt{s}=7$ and $8$ TeV in the ATLAS experiment

Combined analyses of the Higgs boson production and decay rates as well as its coupling strengths to vector bosons and fermions are presented. The combinations include the results of the analyses of the $H\to\gamma\gamma,\, ZZ^*,\, WW^*,\, Z\gamma,\, b\bar{b},\, \tau\tau$ and $\mu\mu$ decay modes, and the constraints on the associated production with a pair of top quarks and on the off-shell coupling strengths of the Higgs boson. The results are based on the LHC proton-proton collision datasets, with integrated luminosities of up to 4.7 $\mathrm{fb}^{-1}$ at $\sqrt{s}=7$ TeV and 20.3 $\mathrm{fb}^{-1}$ at $\sqrt{s}=8$ TeV, recorded by the ATLAS detector in 2011 and 2012. Combining all production modes and decay channels, the measured signal yield, normalised to the Standard Model expectation, is $1.18^{+0.15}_{-0.14}$. The observed Higgs boson production and decay rates are interpreted in a leading-order coupling framework, exploring a wide range of benchmark coupling models both with and without assumptions on the Higgs boson width and on the Standard Model particle content in loop processes. The data are found to be compatible with the Standard Model expectations for a Higgs boson at a mass of 125.36 GeV for all models considered.

==> 05_CouplingFits_custodial.tex <==
\section{Probing the custodial symmetry of the $W$ and $Z$ couplings}
\label{sec:CW/CZ,CF/CZ,CZ2/CH}

{\em This dedicated model for probing the custodial symmetry is retained for historical comparison~\cite{Aad:2013wqa}.
The generic model Section~\ref{sec:gen2} also tests custodial symmetry with fewer assumptions
and a comparable precision and yields consistent results and is considered to be the main result.}

Identical coupling scale factors for the $W$ and $Z$ boson are
required within tight bounds by the $\mathrm{SU(2)}$ custodial
symmetry and the $\rho$ parameter measurements at LEP and at the
Tevatron~\cite{ALEPH:2010aa}. To test this constraint directly in the
Higgs sector, the ratio $\Rr_{\PW\PZ} =\Cc_{\PW}/\Cc_{\PZ}$ is
probed. For the other parameters the same assumptions as in
Section~\ref{sec:bm:CF,CV} on $\Cc_F$ are made ($\Cc_F = \Cc_{\PQt} =
\Cc_{\PQb} = \Cc_{\PGt} = \Cc_{\PGm}$).  The free parameters are:

\begin{eqnarray*}
  \Rr_{\PW\PZ} &=& \Cc_{\PW} / \Cc_{\PZ} \label{kWZ}\\
  \Rr_{FZ} &=& \Cc_F / \Cc_{\PZ} \label{kFZ} \\
  \Cc_{\PZ\PZ} &=& \Cc_{\PZ} \cdot \Cc_{\PZ} / \Cc_{\PH} \label{kZZ} .
\end{eqnarray*}


The ratio $\Rr_{\PW\PZ}$ is in part directly constrained by the decays
in the \hWWlnln\ and \hZZllll\ channels and the $WH$ and $ZH$
production processes.  It is also indirectly constrained by the VBF
production process, which in the SM is $74\%$ $W$ fusion and $26\%$
$Z$ fusion-mediated (see Table \ref{tab:kexpr}).  The scale
factor $\Cc_W$ is also constrained by the \hgg\ channel since the
decay branching ratio receives a dominant contribution from the $W$
loop. Figure~\ref{fig:bm:CW/CZ,CF/CZ,CZ2/CH} shows the profile 
likelihood ratio curve as a function of $\Rr_{\PW\PZ}$. 



\begin{figure}[htbp]
  \center
  \includegraphics[width=.50\textwidth]{figure_scan_custodial_RCWCZ}
  \caption{Results of fits for the benchmark model
    that probe the custodial symmetry through the ratio $\Rr_{\PW\PZ} = \Cc_{\PW} /
    \Cc_{\PZ}$ ($\Rr_{F\PZ}$ and $\Cc_{\PZ\PZ}$ are profiled); The dashed curves show the SM expectations.
    The red (green) horizontal line indicates the value on the profile likelihood ratio corresponding to a 68\% (95\%) confidence interval on the parameter of interest, assuming the asymptotic $\chi^2$ distribution for the test statistic.
    \label{fig:bm:CW/CZ,CF/CZ,CZ2/CH}
  }
\end{figure}

The fit prefers the SM-like local minimum with a positive sign for
$\Rr_{F\PZ}$, implying a positive relative sign between the fermion
and Z couplings

The fit results for the parameters of interest, when profiling the other parameters, are:
\begin{eqnarray*}
    \Rr_{\PW\PZ} &=& \RESULTmodelCUSTvalueRWZ\\
    \Rr_{F\PZ} &=& \RESULTmodelCUSTvalueRFZ\\
    \Cc_{\PZ\PZ} &=& \RESULTmodelCUSTvalueCZZ .
\end{eqnarray*}
The three-dimensional compatibility of the SM hypothesis with the
best-fit point is $\RESULTmodelCUSTpvalueSM$.


